Realms: A Structure for Consolidating Knowledge about Mathematical Theories

Since there are different ways of axiomatizing and developing a mathematical theory, knowledge about a such a theory may reside in many places and in many forms within a library of formalized mathematics. We introduce the notion of a realm as a structure for consolidating knowledge about a mathematical theory. A realm contains several axiomatizations of a theory that are separately developed. Views interconnect these developments and establish that the axiomatizations are equivalent in the sense of being mutually interpretable. A realm also contains an external interface that is convenient for users of the library who want to apply the concepts and facts of the theory without delving into the details of how the concepts and facts were developed. We illustrate the utility of realms through a series of examples. We also give an outline of the mechanisms that are needed to create and maintain realms.

==> pgflibrarytikzmmt.code.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% A TIKZ library for MMT Theory Graphs
% copyright 2014 Michael Kohlhase; Released under the LPPL
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% this library provides some standardized node and arrow styles for formatting MMT graph
% diagrams in tikz. The advantage is that we can classify the arrows and nodes
% symbolically and with the styles in this library achieve a uniform look that helps
% readability. 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% 1. Theories
% a generic theory
\tikzstyle{thy}=[draw,outer sep=.6mm,rounded corners]
% a primitive theory
\tikzstyle{primthy}=[thy,double]
% a theory graph 
\tikzstyle{thygraph}=[draw,outer sep=1mm,rounded corners,dashed]

%%% 2. Arrows 
%%% 2.1. Arrowtips (only internal)
\usetikzlibrary{arrows}
\newcommand{\@mmtarrowtip}{angle 45}
\newcommand{\@mmtreversearrowtip}{angle 45 reversed}
\newcommand{\@mmtarrowtipepi}{triangle 45}
\newcommand{\@mmtarrowtipmonoright}{right hook}
\newcommand{\@mmtarrowtipmonoleft}{left hook}
\newcommand{\@mmtarrowtippartial}{right to}
\newcommand{\@mmtarrowtippartialleft}{left to}
\newcommand{\@mmtreversearrowtippartial}{right to reversed}
\newcommand{\@mmtreversearrowtippartialleft}{left to reversed}

%%% 1.2 the arrow sstyles in graphs
\usetikzlibrary{decorations,decorations.pathmorphing}
% any morphism 
\tikzstyle{morph}=[-\@mmtarrowtip] 
\tikzstyle{mapsto}=[|-\@mmtarrowtip] %| any morphism 
% structures
\tikzstyle{struct}=[-\@mmtarrowtip,thick]
% inclusions: regular, partial, and left variants
\tikzstyle{include}=[\@mmtarrowtipmonoright-\@mmtarrowtip,thick]
\tikzstyle{pinclude}=[\@mmtarrowtipmonoright-\@mmtarrowtippartial,thick]
\tikzstyle{includeleft}=[\@mmtarrowtipmonoleft-\@mmtarrowtip,thick]
\tikzstyle{pincludeleft}=[\@mmtarrowtipmonoleft-\@mmtarrowtippartialleft,thick]
% views: regular, mono, partial, and left variants
\tikzstyle{preview}=[decorate,
                                decoration={coil,aspect=0,amplitude=1pt,
                                                    segment length=6pt,
                                                    pre=lineto,pre length=5pt,
                                                    post=lineto,post length=7pt},
                                thick]
\tikzstyle{view}=[preview,-\@mmtarrowtip]
\tikzstyle{mview}=[preview,\@mmtarrowtipmonoright-\@mmtarrowtip]
\tikzstyle{pview}=[preview,-\@mmtarrowtippartial]
\tikzstyle{pmview}=[preview,\@mmtarrowtipmonoright-\@mmtarrowtippartial]
\tikzstyle{viewleft}=[preview,-\@mmtarrowtip]
\tikzstyle{mviewleft}=[preview,\@mmtarrowtipmonoleft-\@mmtarrowtip]
\tikzstyle{pviewleft}=[preview,-\@mmtarrowtippartialleft]
\tikzstyle{pmviewleft}=[preview,\@mmtarrowtipmonoleft-\@mmtarrowtippartialleft]
% biviews: regular, partial, and left variants
\tikzstyle{biview}=[preview,\@mmtreversearrowtip-\@mmtarrowtip]
\tikzstyle{pbiview}=[preview,\@mmtreversearrowtippartial-\@mmtarrowtippartial]
\tikzstyle{pbiviewleft}=[preview,\@mmtreversearrowtippartialleft-\@mmtarrowtippartialleft]
% defining views (experimental)
\tikzstyle{defview}=[preview,double,-\@mmtarrowtip]
% meta-theory inclusion
\tikzstyle{meta}=[dotted,-\@mmtarrowtip,thick]
% conservative extensions (abbreviation)
\tikzstyle{conservative}=[hooks-\@mmtarrowtip,double] 
% conservative development
\tikzstyle{conservdev}=[hooks-\@mmtarrowtip,dashed,double] 

%%% 3. convenience macros
%%% 3.1 the \mmtthy macro takes three arguments, name, decl, axioms and makes a 
% table-like structure
\newcommand\mmtthy[3]{\def\@test{#3}%
\begin{array}{l}\textsf{#1}\\\hline #2\ifx\@test\@empty\else\\\hline #3\fi\end{array}}
%%% 3.2 the \mmtar takes two arguments, some tikz options, and an arrow style. \nmmtar
% is a variant that also has a name on top.
\newcommand\mmtar[2][]{\raisebox{.5ex}{\tikz[#1]{\draw[#2] (0,0) -- (.6,0);}}}
\newcommand\nmmtar[3][]{\raisebox{.4ex}{\tikz[#1]{\draw[#2] (0,0) --
      node[above]{\ensuremath{\scriptstyle #3}} (.8,0);}}}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "note"
%%% End: 



==> tikzlibrarymmt.code.tex <==
\input{pgflibrarytikzmmt.code.tex}

